Multilingual Twitter Corpus and Baselines for Evaluating Demographic Bias in Hate Speech Recognition

Existing research on fairness evaluation of document classification models mainly uses synthetic monolingual data without ground truth for author demographic attributes. In this work, we assemble and publish a multilingual Twitter corpus for the task of hate speech detection with inferred four author demographic factors: age, country, gender and race/ethnicity. The corpus covers five languages: English, Italian, Polish, Portuguese and Spanish. We evaluate the inferred demographic labels with a crowdsourcing platform, Figure Eight. To examine factors that can cause biases, we take an empirical analysis of demographic predictability on the English corpus. We measure the performance of four popular document classifiers and evaluate the fairness and bias of the baseline classifiers on the author-level demographic attributes.

==> README <==
KNOWN ISSUES

Even if the compilation is successful, on overleaf the following error message appears during (re)compilation:
===ERROR MESSAGE BEGINNING===
 /usr/local/texlive/2018/texmf-dist/tex/latex/base/ts1enc.dfu, line 115
Missing number, treated as zero.

<to be read again> 
                   F
l.115 ...icodeCharacter{FEFF}{\ifhmode\nobreak\fi}
                                                  
A number should have been here; I inserted `0'.
(If you can't figure out why I needed to see a number,
look up `weird error' in the index to The TeXbook.)
===ERROR MESSAGE END===

